Spin decoherence in VOPc@graphene nanoribbon complexes

Carbon nanoribbon or nanographene qubit arrays can facilitate quantum-to-quantum transduction between light, charge, and spin, making them an excellent testbed for fundamental science in quantum coherent systems and for the construction of higher-level qubit circuits. In this work, we study spin decoherence due to coupling with a surrounding nuclear spin bath of an electronic molecular spin of a vanadyl phthalocyanine (VOPc) molecule integrated on an armchair-edged graphene nanoribbon (GNR). Density functional theory (DFT) is used to obtain ground state atomic configurations. Decay of spin coherence in Hahn echo experiments is then simulated using the cluster correlation expansion method with a spin Hamiltonian involving hyperfine and electric field gradient tensors calculated from DFT. We find that the decoherence time $T_2$ is anisotropic with respect to magnetic field orientation and determined only by the hydrogen nuclear spins both on VOPc and GNR. Large electron spin echo envelope modulation (ESEEM) due to nitrogen and vanadium nuclear spins is present at specific field ranges and can be completely suppressed by tuning the magnetic field. The relation between these field ranges and the hyperfine interactions is analyzed. The effects of interactions with the nuclear quadrupole moments are also studied, validating the applicability and limitations of the spin Hamiltonian when they are disregarded.

==> qmdefs.tex <==
% Derivatives
\def\dx{{\partial \over \partial x}}
\def\dy{{\partial\over\partial y}}
\def\dz{{\partial\over\partial z}}
\def\dxx{{\partial^2\over\partial x^2}}
\def\dyy{{\partial^2\over\partial y^2}}
\def\dzz{{\partial^2\over\partial z^2}}
\def\Dx#1{{\partial #1\over \partial x}}
\def\Dy#1{{\partial #1\over \partial y}}
\def\Dz#1{{\partial #1\over \partial z}}
\def\Dzz#1{{\partial^2 #1\over \partial z^2}}
\def\Dyy#1{{\partial^2 #1\over \partial y^2}}
\def\Dxx#1{{\partial^2 #1\over \partial x^2}}
\def\Dt#1{{\partial #1 \over \partial t}}
\def\dphi{{\partial\over\partial \phi}}
\def\dth{{\partial\over\partial \theta}}
\def\dr{{\partial\over \partial r}}
\def\Dphi#1{{\partial #1\over \partial \phi}}
\def\Dth#1{{\partial #1\over \partial \theta}}
\def\Dr#1{{\partial #1\over \partial r}}
\def\Drr#1{{\partial^2 #1\over\partial r^2}}
\def\dt{{\partial\over \partial t}}
\def\dert{{d\over dt}}
\def\dtau{{\partial\over \partial \tau}}
\def\Dtau#1{{\partial #1\over \partial\tau}}
\def\Dert#1{{d #1\over d t}}
\def\Derx#1{{d #1\over d x}}
\def\Derrr#1{{d^2 #1\over d r^2}}
\def\Derr#1{{d #1\over dr}}
\def\derx{{d\over dx}}
% Bolds
\def\k{{\bf k}}
\def\r{{\bf r}}
\def\R{{\bf R}}
\def\q{{\bf q}}
\def\p{{\bf p}}
\def\x{{\bf x}}
\def\yvec{{\bf y}}
\def\xvec{{\bf x}}
\def\rvec{{\bf r}}
\def\qvec{{\bf q}}
\def\kvec{{\bf k}}
\def\pvec{{\bf p}}
\def\pvh{{\hat{\bf p}}}
\def\jvec{{\bf j}}
\def\Avec{{\bf A}}
\def\Bvec{{\bf B}}
\def\Evec{{\bf E}}
\def\Fvec{{\bf F}}
\def\Lvec{{\bf L}}
\def\Jvec{{\bf J}}
\def\Pvec{{\bf P}}
\def\Rvec{{\bf R}}
\def\Svec{{\bf S}}
\def\dvec{{\bf d}}
\def\vvec{{\bf v}}
% Hats
\def\ih{{\hat i}}
\def\jh{\hat j}
\def\kh{\hat k}
\def\hatn{\hat n}
\def\hath{{\hat h}}
\def\hatA{{\hat A}}
\def\hatB{{\hat B}}
\def\hatC{{\hat C}}
\def\hatD{{\hat D}}
\def\hatF{{\hat F}}
\def\hatH{{\hat H}}
\def\hatJ{{\hat J}}
\def\hatK{{\hat K}}
\def\hatL{{\hat L}}
\def\hatS{{\hat S}}
\def\hatV{{\hat V}}
\def\hatQ{\hat Q}
\def\hatp{\hat p}
\def\hatP{\hat P}
\def\hatO{\hat O}
\def\O{\hat{\cal O}}
\def\hatr{{\hat r}}
\def\hatT{{\hat T}}
\def\hatU{\hat U}
\def\hatN{\hat N}
\def\rvh{{\hat{\bf r}}}
\def\hatpsi{{\hat\psi}}
\def\hatrho{{\hat\rho}}
\def\hatpsidag{{\hat\psi}^\dagger}
% Bras and kets
\def\psiket{|\psi\rangle}
\def\psibra{\langle\psi |}
\def\phiket{|\phi\rangle}
\def\phibra{\langle\phi |}
\def\xket{|x\rangle}
\def\xbra{\langle x |}
\def\pket{|{\bf p}\rangle}
\def\pbra{\langle {\bf p} |}
\def\rket{|{\bf r}\rangle}
\def\nket{| n\rangle}
\def\nbra{\langle n |}
\def\mket{| m\rangle}
\def\mbra{\langle m |}
\def\rbra{\langle {\bf r} |}
\def\ket#1{|#1\rangle}
\def\bra#1{\langle #1|}
\def\vacket{\ket{0}}
\def\vacbra{\bra{0}}
\def\vac{\vacket}
\def\dket{\ket{\downarrow}}
\def\uket{\ket{\uparrow}}
\def\dbra{\bra{\downarrow}}
\def\ubra{\bra{\uparrow}}
% Math symbols
\def\paulix{\left[\begin{array}{cc}0 & 1\\1 & 0\end{array}\right]}
\def\pauliy{\left[\begin{array}{cc}0&-i\\i&0\end{array}\right]}
\def\pauliz{\left[\begin{array}{cc}1&0\\0&-1\end{array}\right]}
\def\up{\uparrow}
\def\down{\downarrow}
\def\bigint{\displaystyle\int}
\def\Tr{{\rm Tr}}
\def\ve{\varepsilon}
\def\dg#1{#1^\dagger}
\def\adag{a^\dagger}
\def\bdag{b^\dagger}
\def\cdag{c^\dagger}
\def\Adag{A^\dagger}
\def\Bdag{B^\dagger}
\def\Cdag{C^\dagger}
\def\psidag{\psi^\dagger}
% Spacing & layout
\def\sp{\vskip .2cm\noindent}
\def\bsp{\sp\sp}
% Bold operators (hats)
\def\Sop{{\bf{\hat S}}}
\def\Lop{\bf{\hat L}}
\def\Jop{\bf{\hat J}}
% Misc.
\def\T{{\cal T}}
\def\Lz{\hat{L}_z}
\def\Lsq{\hat{L}^2}
\def\pre{-{\hbar^2\over 2m}}
\def\psic{\psi^*}
\def\avg#1{\langle #1 \rangle}
\def\={&=&}
\def\mybox#1{\fbox{\mbox{$\displaystyle #1 $}}}
\def\aks{a_{\k\sigma}}
\def\adks{\adag_{\k\sigma}}
